Two-Loop Integrals for Planar Five-Point One-Mass Processes

We present the computation of a full set of planar five-point two-loop master integrals with one external mass. These integrals are an important ingredient for two-loop scattering amplitudes for two-jet-associated W-boson production at leading color in QCD. We provide a set of pure integrals together with differential equations in canonical form. We obtain analytic differential equations efficiently from numerical samples over finite fields, fitting an ansatz built from symbol letters. The symbol alphabet itself is constructed from cut differential equations and we find that it can be written in a remarkably compact form. We comment on the analytic properties of the integrals and confirm the extended Steinmann relations, which govern the double discontinuities of Feynman integrals, to all orders in $\epsilon$. We solve the differential equations in terms of generalized power series on single-parameter contours in the space of Mandelstam invariants. This form of the solution trivializes the analytic continuation and the integrals can be evaluated in all kinematic regions with arbitrary numerical precision.

==> notation.tex <==
% !TEX root = main.tex




\section{Scattering kinematics}
\label{sec:scatKin}

The main goal of this paper is the calculation of a basis of two-loop integrals
relevant for planar five-point scattering processes with a single massive
external leg. However, before we delve into that problem, we first briefly 
discuss the kinematics of these processes and introduce some quantities that will
be relevant in the following sections.



The momenta of the scattering particles are labelled $p_i$, $i=1,\ldots,5$, and
fulfil momentum conservation, $\sum_{i=1}^5 p_i =0$. 
Without loss of generality, we assume $p_1$ to be massive, 
i.e.~$p_1^2 = \offShellScale{}$, and the remaining ones to be
massless, $p_{i}^2=0$ for  $i=2,\ldots,5$. 
Out of these momenta,  we can form six independent Mandelstam variables
of the form  $s_{ij}=(p_i+p_j)^2$, which we choose to be
\begin{equation} \label{eqn:orderedInvariants}
\vec s= \{ \offShellScale{} \,,
s_{12}\,, s_{23}\,,s_{34}\,, s_{45}\,, s_{51}\}\,.
\end{equation}
For concreteness, in this paper we use the metric $g = \mathrm{diag}(+,-,-,-)$.
These variables are not sufficient to describe the kinematics of the scattering
process: there is an additional discrete parity which can be
specified by the parity-odd Levi-Civita contraction
\begin{equation}
\label{eq:tr5}
\trFive{} = 4 i \varepsilon_{\alpha\beta\gamma\delta} 
\,p_1^\alpha p_2^\beta p_3^\gamma p_4^\delta\,.
\end{equation}
Indeed, space-time parity inverts all spatial momentum components,
\begin{equation}
 P:\quad ( p_i^0, \vec p_i )\quad \rightarrow \quad ( p_i^0, -\vec p_i )\,,
\end{equation}
and, while Mandelstam variables are invariant,
$\trFive{}$ gains a sign under this transformation. 


Gram determinants are useful when discussing kinematics of scattering
processes. They are computed as the determinants of the
Gram matrix $G(q_1,\ldots,q_n)$, which is defined as
\begin{equation}\label{eq:gramGen}
	G(q_1,\ldots,q_n)=2\,V^T(q_1,\ldots,q_{n-1})\,g\,V(q_1,\ldots,q_{n-1})
	=2 \, \{q_i\cdot q_j\}_{i,j\in\{1,\ldots,n-1\}}\,,
\end{equation}
where the factor of two is conventional and $V(q_1,\ldots,q_{n-1})$ is 
a 4-by-$(n-1)$ matrix whose columns are the vectors $q_i$.
It is clear from the definition of the Gram matrix that the Gram determinant
vanishes if the $q_i$ are not linearly independent, and that it is
invariant under shifts of any of the $q_i$ by any of the other momenta.
In particular, the choice of which momentum does not appear in $V$, 
momentum $q_n$ in our case, is purely conventional.
Returning to the discussion of five-point one-mass kinematics, we note that
the parity-odd $\trFive{}$ is related to the parity-even five-point Gram 
determinant through
\begin{equation}
	\label{eq:gram5}
	\Delta_5 =  \det G(p_1,p_2,p_3,p_4)=\det \{2\, p_i\cdot p_j \}_{i,j\in\{1,2,3,4\}}=
	\textrm{tr}_5^2\,.
\end{equation}
In other words, $\trFive{}$ is a square-root of a polynomial
in the Mandelstam variables $\vec s$.
Two other square-roots related to Gram determinants which are not perfect squares
are relevant for the scattering kinematics we are considering. 
They can be seen to appear already
when five-point one-mass kinematics degenerate to
three-point three-mass kinematics.
The associated Gram determinants can be written in terms 
of the K\"all\'en function $\lambda(a,b,c)$:
% Beyond this, we introduce two objects related to three-point Gram determinants
% by an overall sign. These occur naturally in our scatering kinematics and are
% necessary for both the definition of our basis of integrals, as well as their
% evaluation. They can naturally be written in terms of the K\"all\'en function
% $\lambda$ and are given by
% \draftnote{BP: Rewrite in terms of master Gram and check:}
%
\begin{align}
\label{eq:gram3}
%
\Delta_3&=-\det G(p_1,p_2+p_3,p_4+p_5)
% =-{\rm det} \left(\begin{array}{cc} 2 \offShellScale{} & 2 p_1\!\cdot\!(p_2+p_3)\\
% 		2 p_1\!\cdot\!(p_2+p_3) & 2 (p_2+p_3)^2 
% \end{array}\right) 
= \lambda(\offShellScale{}, s_{23},s_{45}) \,,\\[2ex]
%
\label{eq:gram3NP}
\Delta_3^{\ncg}&=-\det G(p_1,p_3+p_4,p_2+p_5)
% =-{\rm det} \left(\begin{array}{cc} 2 \offShellScale{}  & 2 p_1\!\cdot\!(p_3+p_4)\\
% 		2 p_1\!\cdot\!(p_3+p_4) & 2 (p_3+p_4)^2 
% \end{array}\right) 
= \lambda(\offShellScale{},s_{25},s_{34})\,, \\[2ex]
%
\lambda(a,b,c)&=a^2+b^2+c^2-2ab-2ac-2bc\,,
\end{align}
%
where the minus sign is conventional. Our notation is explained by the fact that
$\Delta_3$ is naturally associated with a degeneration of the
kinematics which preserves the cyclicity of the momenta,
 $\{p_1,p_2,p_3,p_4,p_5\}\to\{p_1,p_2+p_3,p_4+p_5\}$, while 
$\Delta_3^{\ncg}$ is associated with a degeneration that does not preserve it,
$\{p_1,p_2,p_3,p_4,p_5\}\to\{p_1,p_3+p_4,p_2+p_5\}$.

% We note that $\Delta_3$ is present in one-loop scattering amplitudes with a
% cyclic ordering of external legs corresponding to the considered scattering
% kinematics, whereas $\Delta_3^{\rm np}$ is present only in non-cyclic orderings.
% This motivates its labelling. Explicit expressions for Gram determinants are
% given in the ancillary file \texttt{anc/determinants.m}.



% so here depend on $6$ independent parameters, which we specify in terms of the
% Mandelstam invariants $s_{ij}=(p_i+p_j)^2$ in addition to a discrete parity
% label. In this work, we employ the ``mostly minus'' metric $g = \mathrm{diag}(+,
% -, -, -)$. We parametrize the degrees of freedom we with the ordered variables
% %
% \begin{eqnarray} \label{eqn:orderedInvariants}
% \vec s= \{ \offShellScale{} \,,
% s_{12}\,, s_{23}\,,s_{34}\,, s_{45}\,, s_{51}\}\,,
% \end{eqnarray}
% %
% and the parity odd Levi-Civita contraction
% %
% \begin{eqnarray}
% \label{eq:tr5}
% \trFive{} = 4 i \varepsilon_{\alpha\beta\gamma\delta} \,p_2^\alpha p_3^\beta p_4^\gamma p_5^\delta\,
% \end{eqnarray}
% %
% for the parity label.
% Space-time parity inverts all spatial momentum components,
% %
% \begin{eqnarray}
%  P:\quad ( p_i^0, \vec p_i )\quad \rightarrow \quad ( p_i^0, -\vec p_i )\,,
% \end{eqnarray}
% and so $\trFive{}$ gains a sign under parity.
% %


% Importantly, the parity odd $\trFive{}$ can be
% related to the parity even 5-point Gram determinant through
% \begin{align}
% \label{eq:gram5}
% \Delta_5& = (\trFive{})^2 = \det \{ 2 p_i\cdot p_j \}_{i,j=2,5}\,.
% \end{align}


%\subsection{Physical region for vector-boson production at hadron colliders}










% We have in mind the planar processes with the particle ordering $\{1,2,3,4,5\}$. 
% In the Euclidean region, away from all branch cuts, the kinematic invariants
% $\vec s$ take negative values.
%There all Gram determinants are positive and their square roots positive or
%negative. Thus for the above functions we have $\Delta_5>0$ and $\Delta_3^{\rm
%  np},\Delta_3<0$. \draftnote{HI: check this statement: for negative kinematic
%  invariants we can find surfaces of positive and negative $\Delta_3$. }

% An important question when evaluation Feynman integrals
% associated with a scattering process is the kinematic region where
% the integrals are evaluated. 
% When evaluation Feynman integrals associated with a scattering process
% it is important to specify 

% Feynman integrals are multi-valued functions and one must be careful 
% when evaluating at different 


We finish this section by introducing the concept of kinematic
region, which will be useful when we present numerical results for the
integrals we will be computing. Feynman integrals evaluate to functions
of the Mandelstam variables $\vec s$ with a complicated branch-cut structure.
As one moves in the 6-dimensional space of the Mandelstam variables, 
the function will in general be discontinuous if we cross the branch-cuts. 
Each subregion where the function is continuous we call a 
kinematic region. The study of the branch-cut structure of Feynman integrals
is a very rich subject that goes back to the early days of quantum-field
theory\cite{}. The Landau equations \cite{} are a central tool in this study,
as they give a set of necessary conditions for the integrals to have
a branch-point.
For our purpose, it is sufficient to note that the Feynman integrals
we compute have branch-cuts starting at $\offShellScale{}=0$,
$s_{12}=0$, $s_{23}=0$, $s_{34}=0$, $s_{45}=0$ and $s_{15}=0$.
We will thus label different kinematic regions by the sign of the Mandelstam
invariants. We note that not all kinematic regions correspond
to physical scattering configurations (i.e., while we are free
to choose the Mandelstam variables to take any value we wish, some values
do not correspond to physical four-momenta $p_i$).

A particularly relevant region when studying Feynman integrals is 
the Eucledian region, where all the Mandelstam variables are negative
and the integral is real. For five-point one-mass
kinematics, this region is not physical.
%
%
%
% When evaluating Feynman integrals, it is important to specify in which
% kinematic regions the results are valid. \draftnote{Do we say why?}
% In the absence of masses in the propagators, we can label different kinematic regions
% by the sign of the Mandelstam variables $\vec s$. For instance,
% the (non-physical) Eucledian region is defined by having all invariants
% negative. 
A natural application of the two-mass five-point two-loop integrals
is the calculation of the production of a massive vector-boson in association 
with two jets in QCD, so we now briefly discuss the associated kinematic regions.
We assign the massless momenta $p_i\,,i=2,\ldots,5$
to massless partons and the massive momentum $p_1$ to the vector boson,
which we assume then decays into a lepton pair. 
This implies that the momentum $p_1$ is timelike, i.e.~$p_1^2=\offShellScale{}>0$.
%
% We consider the physical region relevant for associated vector-boson production
% in QCD. It is convenient to associate the massless momenta $p_i\,,i=2,..,5$ to
% partons and the massive momentum $p_1$ to a vector boson, which in turn is
% coupled to a lepton pair $p_1=q_\ell+q_{\ell'}$. 
%
Since any of the parton momenta may be in the initial state, we have
six different channels,
\begin{equation}
p_i+p_j \rightarrow p_1+p_k+p_l\,,\quad i,j,k,l\in \{2,3,4,5\}\,,
\end{equation}
and to each corresponds a kinematic region.
In Table~\ref{tab:regions} we give the signs of the kinematic invariants
for each region.
We note that, since momenta corresponding to a physical scattering process must
have real components, it follows from \eqref{eq:gramGen} that 
$\Delta_5<0$ (the sign is determined by the sign of $\det(g)=-1$).

% Finally, the three-point and five-point Gram determinants of
% eqs.~\eqref{eq:gram5}, \eqref{eq:gram3} and \eqref{eq:gram3NP}
% are negative in all physical regions, which implies $\Delta_5<0$ and
% $\Delta_3^{\rm np},\Delta_3>0$. The sign of the determinant $\Delta_5<0$ follows
% from the requirement of real-valued momenta with our convention of metric signature.
% Regarding $\Delta_3$ and $\Delta_3^{\rm np}$, we find that the associated Gram
% determinants are positive if all momenta are spacelike, while they are negative
% if at least one momentum is timelike. \draftnote{This seems wrong}
% The signs of $\Delta_3$ and $\Delta_3^{\rm np}$ can be derived from properties of
% their argument momenta and the associate Gram determinants. These gram
% determinants are positive, if all momenta are spacelike, while they are negative
% if at least one momentum is timelike.
% In fact, in the physical regions we find that at least one of the argument
% momenta is timelike. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{table}[]
\centering
 \begin{tabular}{| c || c | c | c | c | } 
\hline
 process	&  initial state  	& $	>0				$&$	<0			  $\\\hline\hline  
 Euclidean 	& ---			&&	$ s_{12}, s_{23}, s_{34}, s_{45}, s_{15}, \offShellScale{} $		\\ \hline \hline
V-production 	&	$2,3$		& $ s_{23},s_{45},s_{15},\offShellScale $&$ s_{12},s_{34} 	  	  $       			\\ \hline       
	 	&	$2,4$		& $ s_{15},\offShellScale 		$&$ s_{12},s_{23},s_{34},s_{45}   $ 				\\ \hline
	 	&	$2,5$		& $ s_{34},\offShellScale 		$&$ s_{12},s_{23},s_{45},s_{15}   $ 				\\ \hline
	 	&	$3,4$		& $ s_{12},s_{34},s_{15},\offShellScale $&$ s_{23},s_{45} 		  $  	   			\\ \hline
	 	&	$3,5$		& $ s_{12},\offShellScale 		$&$ s_{23},s_{34},s_{45},s_{15}	  $				\\ \hline
	 	&	$4,5$		& $ s_{12},s_{23},s_{45},\offShellScale $&$ s_{34},s_{15}                 $				\\ \hline
  \end{tabular}
 \caption{Signs of first entry Mandelstam invariants in the Euclidean and the physical 
 phase space.  }
 \label{tab:regions}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\draftnote{Check table}














